ModularityCheck: A Tool for Assessing Modularity using Co-Change Clusters

It is widely accepted that traditional modular structures suffer from the dominant decomposition problem. Therefore, to improve current modularity views, it is important to investigate the impact of design decisions concerning modularity in other dimensions, as the evolutionary view. In this paper, we propose the ModularityCheck tool to assess package modularity using co-change clusters, which are sets of classes that usually changed together in the past. Our tool extracts information from version control platforms and issue reports, retrieves co-change clusters, generates metrics related to co-change clusters, and provides visualizations for assessing modularity. We also provide a case study to evaluate the tool. http://youtu.be/7eBYa2dfIS8

==> sections/estadoAtual.tex <==
Specifically, we are investigating a novel approach for assessing modularity, based on co-change graphs~\citep{beyer2005}. The approach is directly inspired by the common criteria used to decompose systems in modules, i.e.,~modules should confine implementation decisions that are likely to change~\citep{parnas72}. We first extract co-change graphs from the history of changes in software systems. In such graphs, the nodes are classes and the edges link classes that were modified together in the same commit transaction.  After that, co-change graphs are automatically processed to produce a new modular facet: co-change clusters, which abstract out common changes made to a system, as stored in version control platforms. Therefore, co-change clusters represent sets of classes that changed together in the past.

Our approach relies on distribution maps~\citep{ducasse2006}---a well-known visualization technique---to reason about the projection of the extracted clusters in the traditional decomposition of a system in packages. We then rely on a set of metrics defined for distribution maps to characterize the extracted co-change clusters. Particularly, we already identified some recurrent distribution patterns of co-change clusters, including patterns denoting well-modularized and crosscutting clusters. Moreover, we also evaluate the meaning of the obtained clusters using information retrieval techniques. The goal in this particular case is to understand how similar are the issues whose commits were clustered together. We already used our approach to assess the modularity of three real-world systems (Geronimo, Lucene, and Eclipse JDT Core) and observed different patterns of co-change modularity in such systems.
For instance, most co-change clusters in Geronimo are well-encapsulated, suggesting that the package's system are well-modularized. In counterpart, the co-change clusters in Lucene contains two types of patterns that may suggest modularity flaws. Several co-change clusters are crosscutting and some represent a pattern that indicate a possible ripple effect during maintenance activities. 
